Timing of stellar pulsations to search for sub-stellar companions beyond the main sequence

(abridged) Stars spend most of their life on the main sequence (MS). But their most substantial changes occur off the MS stage, either before on the pre-MS or beyond at the post-MS phase. Due to very complex and varied dynamical processes, the evolution of planetary systems orbiting non-MS stars significantly differs from those of MS planetary systems. This work focusses on the search for sub-stellar companions in post-MS systems146 and determination of the evolutionary state of their host stars, especially subdwarf B stars (sdB stars). The canonical model involves binary evolution to explain the existence of sdB stars. Formation scenarios for single sdBs are more controversially discussed. Besides the merger of two helium white dwarfs or other merger processes for apparently single sdB stars, an alternative formation channel involves planetary systems. During the red giant phase, the star would develop a common envelope w146ith a giant planet that leads to the loss of the envelope. Thus, sdB stars are laboratories to test how planets survive and influence the late phases of stellar evolution. The rapid pulsations of sdB stars can be used to detect sub-stellar companions from periodic variations in the expected arrival times of the pulsation maxima. This timing method is particularly sensitive to companions at large distances and complementary to other exoplanet detection methods. Thus, the timing method opens up a new parameter range in terms of the host stars and helps to understand the formation process of single sdBs. In this work I implemented, tested and applied the pulsation timing analysis to search for sub-stellar companions in late evolutionary stage stellar systems. The method is already established in the literature but not to an extent which is capable of automatically processing long-time series of high-cadence data, i.e., from space born observations.

==> cv.tex <==
\centering
\begin{tabular}{rl}
	{\large \textbf{Personal Details}}\normalsize & \\
	 & \\
	Date of birth &  December 10, 1992 \\
	Place of birth & Brandenburg/Havel \\
	Nationality & German \\
	 & \\
 	 & \\
	{\large \textbf{Education}}\normalsize & \\
	 & \\
	\textbf{PhD student} & \\
	10/2016 -- 4/2020 & \makecell{at the International Max Planck Research School \\for Solar System Science and the University of G\"ottingen} \\
	Thesis & \makecell{Timing of stellar pulsations to search for \\sub-stellar companions beyond the main sequence}\\
	Advisor & Dr. S. Schuh \\
	Thesis Advisory Committee & Dr. S. Schuh, Prof. Dr. L. Gizon, Prof. Dr. S. Dreizler \\
	& \\
	\textbf{M.Sc. in Physics} & \\
	10/2014 - 09/2016 & \makecell{at the University of Potsdam and \\the Leibniz-Institute for Astrophysics Potsdam} \\
	Thesis & \makecell{Transmission spectroscopy of exoplanet atmospheres -- \\ On the Rayleigh-like feature of TrES-3b}\\
	Advisor & Prof. Dr. K. G. Strassmeier, Dr. M. Mallonn, \\
	& \\
	\textbf{B.Sc. in Physics} & \\
	10/2011 - 09/2014 & \makecell{at the University of Potsdam and \\the Leibniz-Institute for Astrophysics Potsdam} \\
	Thesis & \makecell{Detecting planets orbiting the eclipsing polar CSS~081231}\\
	Advisor & Prof. Dr. W.-R. Hamann, Dr. A. Schwope \\
\end{tabular}


==> exotime/dicussion.tex <==
\section{Discussion}\label{sec:discussion}

\subsection{DW Lyn}
%In order to determine evolutionary timescales of the pulsations we investigate the long term evolution in the $ O-C $-data. A constant change in period results in a second order term as a function of time, which allows us to derive a value for the secular change of the period $ \dot{P} $ and hence the evolutionary time scale. Results of the fits of the second order polynomial are included into Fig.~\ref{fig:dwlyn-oc}, which are $ \dot{P}/P_{f1} = \left( -1.1 \pm 0.6 \right) \times \unit[10^{-5}]{d^{-1}} $ and $ \dot{P}/P_{f2} = \left( -10.0 \pm 3.0 \right) \times \unit[10^{-5}]{d^{-1}} $. %For $ f_1 $ the change in period differs not from the null hypothesis and for $ f_2 $ by $ \unit[1.4]{\sigma} $. Thus, we consider the pulsations are stable in frequency within the time of our observing campaign. 
%
%After subtracting the long term trend, the feature interpretation on smaller time scales appears to be more puzzling. The $ O-C $-data for $ f_2 $ show a oscillating behaviour with a significance of $ \unit[3]{\sigma} $ within the first 200 days, while the arrival times for $ f_1 $ remain constant. For later epochs the $ O-C $-data for both frequencies agree mostly within $ \unit[1]{\sigma} $ to each other.
%Additionally, the evolution of the pulsation-amplitudes in Fig.~\ref{fig:dwlyn-ampl} shows a similar oscillating behaviour for $ f_2 $ within the first epochs like in the arrival times. The occurrence of phase- and amplitude-modulations indicates a mode-beating of two close frequencies, as already suspected from the residuals of the amplitude spectrum in Fig.~\ref{fig:dwlyn-power}. For later observations the amplitude remains almost constant within the uncertainties. The amplitude for the $ f_1 $ pulsation drops by about 0.4 per cent (amplitude) or about 15 per cent (relative) in the second half of the observation campaign. For both frequencies a possible interaction between pulsation-amplitude and -phase is not well understood. 

%Fig.~\ref{fig:dwlyn-power-planet} shows the amplitude spectra of the arrival times for $ f_1 $ and $ f_2 $ after subtracting the respective change in period. The $ O-C $-data show no simultaneous peaks above the $ \unit[5]{\sigma} $ threshold, indicating no presence of a companion within data set. Additionally, mode-beating is likely to introduce a periodic behaviour in the $ O-C $-diagram. Nevertheless, a companion orbiting with a period longer than half of our observational base line, e.g. longer than $ \unit[\sim600]{d} $, or shorter than our resolution in time, e.g. a couple of days to weeks, are not detectable.
%
%\begin{figure}[htbp!]
%	\centering
%	\input{figures/dwlyn/oc-data/powerspec-planet.tex}
%	\caption{Amplitude $ A_{ltt} $ spectrum of the arrival times for DW Lyn with the $ \unit[5]{\sigma} $ confidence level as dashed line.}
%	\label{fig:dwlyn-power-planet}
%\end{figure}

\subsection{V1636 Ori}
%In the case of V1636 Ori the data quality is not sufficient to model the frequency triplet at $ \unit[631.73]{d^{-1}} $ with high accuracy simultaneously but only the central frequency. Nevertheless, we show that the nature of the $ O-C $-variations emerge most likely due to frequency-beating in combination with the limited time resolution of the data. Simulating three frequencies but analysing only one of them leads to $ O-C $-data in Fig.~\ref{fig:v1636ori-sim}. Except for the very first $ O-C $-value, observations and simulation agree within $ \unit[2.5]{\sigma} $.
%
%Since the apparent behaviour in arrival times of $ f_{1.1} $ can be explained by these simulations, $ f_2 $ remains for an analysis of the evolutionary time scales of the pulsations. The fitted result of the second order polynomial in time is included in Fig.~\ref{fig:v1636ori-oc} and implies a change in period of $ \dot{P}/P_{f2} = \left( 6.4 \pm 6.0 \right)\times \unit[10^{-5}]{d^{-1}} $.
%The amplitudes of the two investigated pulsations in Fig.~\ref{fig:v1636ori-ampl} remain constant within the uncertainties for the range of our observations.
%
%Since we can use only one stellar pulsation frequency for the $ O-C $-analysis, a cross check for signals induced by sub-stellar companions is not possible. Thus, the by \citet{lutz_search_2011} predicted periodicity at $ \unit[160]{d} $ can not be confirmed and is likely to be an artefact induced by the three close frequencies $ f_{1.n} $. This leaves the arrival times of $ f_2 $ for an amplitude spectrum analysis. Fig.~\ref{fig:v1636ori-power-planet} shows multiple peaks above the $ \unit[5]{\sigma} $ threshold. 



==> figures/exotime/dwlyn/amplitudes.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$1.4$}}%
      \csname LTb\endcsname%
      \put(645,952){\makebox(0,0)[r]{\strut{}$1.6$}}%
      \csname LTb\endcsname%
      \put(645,1236){\makebox(0,0)[r]{\strut{}$1.8$}}%
      \csname LTb\endcsname%
      \put(645,1519){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(645,1802){\makebox(0,0)[r]{\strut{}$2.2$}}%
      \csname LTb\endcsname%
      \put(645,2085){\makebox(0,0)[r]{\strut{}$2.4$}}%
      \csname LTb\endcsname%
      \put(645,2369){\makebox(0,0)[r]{\strut{}$2.6$}}%
      \csname LTb\endcsname%
      \put(645,2652){\makebox(0,0)[r]{\strut{}$2.8$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$3$}}%
      \csname LTb\endcsname%
      \put(1279,409){\makebox(0,0){\strut{}$54500$}}%
      \csname LTb\endcsname%
      \put(2043,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(2807,409){\makebox(0,0){\strut{}$55500$}}%
      \csname LTb\endcsname%
      \put(3570,409){\makebox(0,0){\strut{}$56000$}}%
      \csname LTb\endcsname%
      \put(4334,409){\makebox(0,0){\strut{}$56500$}}%
      \csname LTb\endcsname%
      \put(4510,669){\makebox(0,0)[l]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(4510,952){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4510,1236){\makebox(0,0)[l]{\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(4510,1519){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(4510,1802){\makebox(0,0)[l]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(4510,2085){\makebox(0,0)[l]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(4510,2369){\makebox(0,0)[l]{\strut{}$0.7$}}%
      \csname LTb\endcsname%
      \put(4510,2652){\makebox(0,0)[l]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(4510,2935){\makebox(0,0)[l]{\strut{}$0.9$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_1)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(5010,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_2)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2577,130){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}}$}}%
      \csname LTb\endcsname%
      \put(3546,2768){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(3546,2582){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/dwlyn/amplitudes}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/epoch/test.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,5100.00)%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(204,4914){\makebox(0,0)[l]{\strut{}cairolatex  terminal test}}%
      \put(204,4681){\makebox(0,0)[l]{\strut{}gnuplot version 5.0.3  }}%
      \put(1530,2550){\makebox(0,0)[l]{\strut{}12345678901234567890}}%
      \put(1530,2810){\makebox(0,0)[l]{\strut{}test of character width:}}%
      \put(2550,3666){\makebox(0,0)[l]{\strut{}left justified}}%
      \put(2550,3480){\makebox(0,0){\strut{}centre+d text}}%
      \put(2550,3294){\makebox(0,0)[r]{\strut{}right justified}}%
      \put(186,2550){\rotatebox{-270}{\makebox(0,0){\strut{}rotated ce+ntred text}}}%
      \put(558,2550){\rotatebox{45}{\makebox(0,0)[l]{\strut{} rotated by +45 deg}}}%
      \put(372,2550){\rotatebox{-45}{\makebox(0,0)[l]{\strut{} rotated by -45 deg}}}%
      \put(2448,4914){\makebox(0,0)[r]{\strut{}show ticscale}}%
      \csname LTb\endcsname%
      \put(4312,4914){\makebox(0,0)[r]{\strut{}-1}}%
      \csname LTa\endcsname%
      \put(4312,4728){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.58,0.00,0.83}%
      \put(4312,4542){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.00,0.62,0.45}%
      \put(4312,4356){\makebox(0,0)[r]{\strut{}2}}%
      \colorrgb{0.34,0.71,0.91}%
      \put(4312,4170){\makebox(0,0)[r]{\strut{}3}}%
      \colorrgb{0.90,0.62,0.00}%
      \put(4312,3984){\makebox(0,0)[r]{\strut{}4}}%
      \colorrgb{0.94,0.89,0.26}%
      \put(4312,3798){\makebox(0,0)[r]{\strut{}5}}%
      \colorrgb{0.00,0.45,0.70}%
      \put(4312,3612){\makebox(0,0)[r]{\strut{}6}}%
      \colorrgb{0.90,0.12,0.06}%
      \put(4312,3426){\makebox(0,0)[r]{\strut{}7}}%
      \colorrgb{0.00,0.00,0.00}%
      \put(4312,3240){\makebox(0,0)[r]{\strut{}8}}%
      \colorrgb{0.58,0.00,0.83}%
      \put(4312,3054){\makebox(0,0)[r]{\strut{}9}}%
      \colorrgb{0.00,0.62,0.45}%
      \put(4312,2868){\makebox(0,0)[r]{\strut{}10}}%
      \colorrgb{0.34,0.71,0.91}%
      \put(4312,2682){\makebox(0,0)[r]{\strut{}11}}%
      \colorrgb{0.90,0.62,0.00}%
      \put(4312,2496){\makebox(0,0)[r]{\strut{}12}}%
      \colorrgb{0.94,0.89,0.26}%
      \put(4312,2310){\makebox(0,0)[r]{\strut{}13}}%
      \colorrgb{0.00,0.45,0.70}%
      \put(4312,2124){\makebox(0,0)[r]{\strut{}14}}%
      \colorrgb{0.90,0.12,0.06}%
      \put(4312,1938){\makebox(0,0)[r]{\strut{}15}}%
      \colorrgb{0.00,0.00,0.00}%
      \put(4312,1752){\makebox(0,0)[r]{\strut{}16}}%
      \colorrgb{0.58,0.00,0.83}%
      \put(4312,1566){\makebox(0,0)[r]{\strut{}17}}%
      \colorrgb{0.00,0.62,0.45}%
      \put(4312,1380){\makebox(0,0)[r]{\strut{}18}}%
      \colorrgb{0.34,0.71,0.91}%
      \put(4312,1194){\makebox(0,0)[r]{\strut{}19}}%
      \colorrgb{0.90,0.62,0.00}%
      \put(4312,1008){\makebox(0,0)[r]{\strut{}20}}%
      \colorrgb{0.94,0.89,0.26}%
      \put(4312,822){\makebox(0,0)[r]{\strut{}21}}%
      \colorrgb{0.00,0.45,0.70}%
      \put(4312,636){\makebox(0,0)[r]{\strut{}22}}%
      \colorrgb{0.90,0.12,0.06}%
      \put(4312,450){\makebox(0,0)[r]{\strut{}23}}%
      \colorrgb{0.00,0.00,0.00}%
      \put(4312,264){\makebox(0,0)[r]{\strut{}24}}%
      \put(892,204){\makebox(0,0)[l]{\strut{}  lw 1}}%
      \put(892,408){\makebox(0,0)[l]{\strut{}  lw 2}}%
      \put(892,612){\makebox(0,0)[l]{\strut{}  lw 3}}%
      \put(892,816){\makebox(0,0)[l]{\strut{}  lw 4}}%
      \put(892,1020){\makebox(0,0)[l]{\strut{}  lw 5}}%
      \put(892,1224){\makebox(0,0)[l]{\strut{}  lw 6}}%
      \put(382,1428){\makebox(0,0)[l]{\strut{}linewidth}}%
      \csname LTb\endcsname%
      \put(2040,204){\makebox(0,0)[l]{\strut{}  dt 1}}%
      \csname LTb\endcsname%
      \put(2040,408){\makebox(0,0)[l]{\strut{}  dt 2}}%
      \csname LTb\endcsname%
      \put(2040,612){\makebox(0,0)[l]{\strut{}  dt 3}}%
      \csname LTb\endcsname%
      \put(2040,816){\makebox(0,0)[l]{\strut{}  dt 4}}%
      \csname LTb\endcsname%
      \put(2040,1020){\makebox(0,0)[l]{\strut{}  dt 5}}%
      \put(1530,1224){\makebox(0,0)[l]{\strut{}dashtype}}%
      \put(3439,916){\makebox(0,0){\strut{}pattern fill}}%
      \put(2613,730){\makebox(0,0){\strut{} 0}}%
      \put(2803,730){\makebox(0,0){\strut{} 1}}%
      \put(2993,730){\makebox(0,0){\strut{} 2}}%
      \put(3183,730){\makebox(0,0){\strut{} 3}}%
      \put(3373,730){\makebox(0,0){\strut{} 4}}%
      \put(3563,730){\makebox(0,0){\strut{} 5}}%
      \put(3753,730){\makebox(0,0){\strut{} 6}}%
      \put(3943,730){\makebox(0,0){\strut{} 7}}%
      \put(4133,730){\makebox(0,0){\strut{} 8}}%
      \put(3570,4581){\makebox(0,0){\strut{}filled polygons:}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{test}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/oc-data/oc-obs-model.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2735){\makebox(0,0)[r]{\strut{}$-500$}}%
      \csname LTb\endcsname%
      \put(640,3097){\makebox(0,0)[r]{\strut{}$-400$}}%
      \csname LTb\endcsname%
      \put(640,3459){\makebox(0,0)[r]{\strut{}$-300$}}%
      \csname LTb\endcsname%
      \put(640,3822){\makebox(0,0)[r]{\strut{}$-200$}}%
      \csname LTb\endcsname%
      \put(640,4184){\makebox(0,0)[r]{\strut{}$-100$}}%
      \csname LTb\endcsname%
      \put(640,4546){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1005,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1952,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2899,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3846,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4793,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(882,4987){\makebox(0,0){\strut{}2007}}%
      \csname LTb\endcsname%
      \put(1575,4987){\makebox(0,0){\strut{}2008}}%
      \csname LTb\endcsname%
      \put(2267,4987){\makebox(0,0){\strut{}2009}}%
      \csname LTb\endcsname%
      \put(2958,4987){\makebox(0,0){\strut{}2010}}%
      \csname LTb\endcsname%
      \put(3649,4987){\makebox(0,0){\strut{}2011}}%
      \csname LTb\endcsname%
      \put(4342,4987){\makebox(0,0){\strut{}2012}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(37,3731){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(1122,3088){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(1122,2902){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,868){\makebox(0,0)[r]{\strut{}$-100$}}%
      \csname LTb\endcsname%
      \put(640,1117){\makebox(0,0)[r]{\strut{}$-80$}}%
      \csname LTb\endcsname%
      \put(640,1366){\makebox(0,0)[r]{\strut{}$-60$}}%
      \csname LTb\endcsname%
      \put(640,1615){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(640,1864){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(640,2113){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,2362){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(640,2611){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(1005,484){\makebox(0,0){\strut{}$54500$}}%
      \csname LTb\endcsname%
      \put(1952,484){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(2899,484){\makebox(0,0){\strut{}$55500$}}%
      \csname LTb\endcsname%
      \put(3846,484){\makebox(0,0){\strut{}$56000$}}%
      \csname LTb\endcsname%
      \put(4793,484){\makebox(0,0){\strut{}$56500$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(37,1739){\rotatebox{-270}{\makebox(0,0){\strut{}residuals$\unit[/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2804,205){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}-2400000}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{oc-obs-model}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/oc-data/powerspec-planet.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(543,669){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(543,935){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(543,1201){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(543,1468){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(543,1734){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(543,2000){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(543,2266){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(543,2533){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(543,2799){\makebox(0,0)[r]{\strut{}$16$}}%
      \csname LTb\endcsname%
      \put(543,3065){\makebox(0,0)[r]{\strut{}$18$}}%
      \csname LTb\endcsname%
      \put(719,409){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1362,409){\makebox(0,0){\strut{}$300$}}%
      \csname LTb\endcsname%
      \put(2006,409){\makebox(0,0){\strut{}$600$}}%
      \csname LTb\endcsname%
      \put(2649,409){\makebox(0,0){\strut{}$900$}}%
      \csname LTb\endcsname%
      \put(3292,409){\makebox(0,0){\strut{}$1200$}}%
      \csname LTb\endcsname%
      \put(3935,409){\makebox(0,0){\strut{}$1500$}}%
      \csname LTb\endcsname%
      \put(4579,409){\makebox(0,0){\strut{}$1800$}}%
      \csname LTb\endcsname%
      \put(719,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1301,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1883,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2465,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3047,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3629,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4211,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4793,3139){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1867){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{ltt}/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2756,130){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(4005,2898){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(4005,2712){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(4150,950){\makebox(0,0)[l]{\strut{}$\unit[5]{\sigma}$}}%
      \csname LTb\endcsname%
      \put(967,2892){\makebox(0,0){\strut{}$\unit[80]{d}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/dwlyn/oc-data/powerspec-planet}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/oc-data/powerspec.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\definecolor{r}{HTML}{e41a1c}
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(10420.00,6440.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,3499){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,3805){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,4111){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,4417){\makebox(0,0)[r]{\strut{}$3$}}%
      \csname LTb\endcsname%
      \put(640,4723){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(640,5029){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%
      \put(640,5335){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(640,5641){\makebox(0,0)[r]{\strut{}$7$}}%
      \csname LTb\endcsname%
      \put(640,5947){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(640,6253){\makebox(0,0)[r]{\strut{}$9$}}%
      \csname LTb\endcsname%
      \put(816,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2366,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3915,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(5465,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(7014,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(8564,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(10113,3239){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(816,6327){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2366,6327){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3915,6327){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(5465,6327){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(7014,6327){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(8564,6327){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(10113,6327){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(343,4876){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{ltt}/]{s}$}}}%
      \csname LTb\endcsname%
      \put(9325,3666){\makebox(0,0)[r]{\strut{}$f_{1.1}$}}%
      \csname LTb\endcsname%
      \put(7014,5289){\makebox(0,0)[l]{\strut{}$\unit[5]{\sigma}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,744){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1137){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,1531){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(640,1924){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(640,2318){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(640,2711){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(640,3105){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(640,3498){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(816,484){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(2366,484){\makebox(0,0){\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(3915,484){\makebox(0,0){\strut{}$400$}}%
      \csname LTb\endcsname%
      \put(5465,484){\makebox(0,0){\strut{}$600$}}%
      \csname LTb\endcsname%
      \put(7014,484){\makebox(0,0){\strut{}$800$}}%
      \csname LTb\endcsname%
      \put(8564,484){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(10113,484){\makebox(0,0){\strut{}$1200$}}%
      \csname LTb\endcsname%
      \put(816,3572){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2366,3572){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3915,3572){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(5465,3572){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(7014,3572){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(8564,3572){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(10113,3572){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(241,2121){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{ltt}/]{s}$}}}%
      \csname LTb\endcsname%
      \put(5464,205){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(9325,911){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(7014,1895){\makebox(0,0)[l]{\strut{}$\unit[5]{\sigma}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{powerspec}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/oc-obs.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$-80$}}%
      \csname LTb\endcsname%
      \put(645,993){\makebox(0,0)[r]{\strut{}$-60$}}%
      \csname LTb\endcsname%
      \put(645,1316){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(645,1640){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(645,1964){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(645,2288){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(645,2611){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%
      \put(821,409){\makebox(0,0){\strut{}$54400$}}%
      \csname LTb\endcsname%
      \put(1483,409){\makebox(0,0){\strut{}$54600$}}%
      \csname LTb\endcsname%
      \put(2145,409){\makebox(0,0){\strut{}$54800$}}%
      \csname LTb\endcsname%
      \put(2807,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(3469,409){\makebox(0,0){\strut{}$55200$}}%
      \csname LTb\endcsname%
      \put(4131,409){\makebox(0,0){\strut{}$55400$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$55600$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2807,130){\makebox(0,0){\strut{}MBJD(TDB)}}%
      \csname LTb\endcsname%
      \put(4005,1022){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(4005,836){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/dwlyn/oc-obs}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/rv/rv.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5102.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(766,401){\makebox(0,0){\strut{}$0.1$}}%
      \put(1577,401){\makebox(0,0){\strut{}$1$}}%
      \put(2387,401){\makebox(0,0){\strut{}$10$}}%
      \put(3197,401){\makebox(0,0){\strut{}$100$}}%
      \put(4008,401){\makebox(0,0){\strut{}$1000$}}%
      \put(2500,71){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \put(488,804){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(488,1099){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(488,1394){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(488,1689){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(488,1983){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(488,2278){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(488,2573){\makebox(0,0)[r]{\strut{}$12$}}%
      \put(488,2868){\makebox(0,0)[r]{\strut{}$14$}}%
      \put(60,1910){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[m \sin i/]{M_{\jupiter}}$}}}%
      \put(4690,804){\makebox(0,0)[l]{\strut{}$1$}}%
      \put(4690,1235){\makebox(0,0)[l]{\strut{}$2$}}%
      \put(4690,1666){\makebox(0,0)[l]{\strut{}$4$}}%
      \put(4690,2097){\makebox(0,0)[l]{\strut{}$8$}}%
      \put(4690,2528){\makebox(0,0)[l]{\strut{}$16$}}%
      \put(4690,2960){\makebox(0,0)[l]{\strut{}$32$}}%
      \put(5020,1910){\rotatebox{-270}{\makebox(0,0){\strut{}$\sigma$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    	\tiny
		\color{cb-red}%
		\put(4180,1500){\makebox(0,0){\strut{}2}}%
		\color{cb-red}%
		\put(3780,1700){\makebox(0,0){\strut{}3}}%
		\color{cb-red}%
		\put(4020,2500){\makebox(0,0){\strut{}4}}%
%      \colorrgb{0.22,0.49,0.72}%
      \color{cb-blue}%
      \put(3700,2300){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(3735,2647){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(3800,2788){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(3890,2699){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(3922,2388){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4118,2988){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4145,2396){\makebox(0,0){\strut{}3.5}}%
%      \colorrgb{0.22,0.49,0.72}%
      \color{cb-blue}%
      \put(3134,2840){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4095,2677){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4108,1966){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4157,1671){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4189,2373){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4010,2951){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
%      \put(4000,2233){\makebox(0,0){\strut{}3.25}}%
%      \colorrgb{0.22,0.49,0.72}%
      \color{cb-blue}%
      \put(3900,2000){\makebox(0,0){\strut{}3.25}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/dwlyn/rv/rv}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/window1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8500.00,5240.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2620){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,3032){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,3444){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,3857){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(640,4269){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,4681){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(1325,4941){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(2132,4941){\makebox(0,0){\strut{}$-0.15$}}%
      \csname LTb\endcsname%
      \put(2940,4941){\makebox(0,0){\strut{}$-0.1$}}%
      \csname LTb\endcsname%
      \put(3748,4941){\makebox(0,0){\strut{}$-0.05$}}%
      \csname LTb\endcsname%
      \put(4556,4941){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(5363,4941){\makebox(0,0){\strut{}$0.05$}}%
      \csname LTb\endcsname%
      \put(6171,4941){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(6979,4941){\makebox(0,0){\strut{}$0.15$}}%
      \csname LTb\endcsname%
      \put(7786,4941){\makebox(0,0){\strut{}$0.2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,3650){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(4555,5219){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2619){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,970){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,1382){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1795){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,2207){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(816,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(1751,298){\makebox(0,0){\strut{}$-0.015$}}%
      \csname LTb\endcsname%
      \put(2686,298){\makebox(0,0){\strut{}$-0.01$}}%
      \csname LTb\endcsname%
      \put(3621,298){\makebox(0,0){\strut{}$-0.005$}}%
      \csname LTb\endcsname%
      \put(4556,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(5490,298){\makebox(0,0){\strut{}$0.005$}}%
      \csname LTb\endcsname%
      \put(6425,298){\makebox(0,0){\strut{}$0.01$}}%
      \csname LTb\endcsname%
      \put(7360,298){\makebox(0,0){\strut{}$0.015$}}%
      \csname LTb\endcsname%
      \put(8295,298){\makebox(0,0){\strut{}$0.02$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1588){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(4555,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/exotime/dwlyn/window1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/dwlyn/window2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1570){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1823){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(640,2076){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,2328){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(640,2581){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(1093,2841){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(1534,2841){\makebox(0,0){\strut{}$-0.15$}}%
      \csname LTb\endcsname%
      \put(1974,2841){\makebox(0,0){\strut{}$-0.1$}}%
      \csname LTb\endcsname%
      \put(2415,2841){\makebox(0,0){\strut{}$-0.05$}}%
      \csname LTb\endcsname%
      \put(2856,2841){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3296,2841){\makebox(0,0){\strut{}$0.05$}}%
      \csname LTb\endcsname%
      \put(3737,2841){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(4177,2841){\makebox(0,0){\strut{}$0.15$}}%
      \csname LTb\endcsname%
      \put(4618,2841){\makebox(0,0){\strut{}$0.2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,2075){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2855,3119){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1569){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,760){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,962){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1165){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,1367){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(816,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(1326,298){\makebox(0,0){\strut{}$-0.015$}}%
      \csname LTb\endcsname%
      \put(1836,298){\makebox(0,0){\strut{}$-0.01$}}%
      \csname LTb\endcsname%
      \put(2346,298){\makebox(0,0){\strut{}$-0.005$}}%
      \csname LTb\endcsname%
      \put(2856,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3365,298){\makebox(0,0){\strut{}$0.005$}}%
      \csname LTb\endcsname%
      \put(3875,298){\makebox(0,0){\strut{}$0.01$}}%
      \csname LTb\endcsname%
      \put(4385,298){\makebox(0,0){\strut{}$0.015$}}%
      \csname LTb\endcsname%
      \put(4895,298){\makebox(0,0){\strut{}$0.02$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1063){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(2855,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/dwlyn/window2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/amplitudes.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(645,993){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(645,1316){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(645,1640){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(645,1964){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(645,2288){\makebox(0,0)[r]{\strut{}$3$}}%
      \csname LTb\endcsname%
      \put(645,2611){\makebox(0,0)[r]{\strut{}$3.5$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(821,409){\makebox(0,0){\strut{}$52000$}}%
      \csname LTb\endcsname%
      \put(1526,409){\makebox(0,0){\strut{}$53000$}}%
      \csname LTb\endcsname%
      \put(2231,409){\makebox(0,0){\strut{}$54000$}}%
      \csname LTb\endcsname%
      \put(2937,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(3642,409){\makebox(0,0){\strut{}$56000$}}%
      \csname LTb\endcsname%
      \put(4382,669){\makebox(0,0)[l]{\strut{}$-1.5$}}%
      \csname LTb\endcsname%
      \put(4382,993){\makebox(0,0)[l]{\strut{}$-1$}}%
      \csname LTb\endcsname%
      \put(4382,1316){\makebox(0,0)[l]{\strut{}$-0.5$}}%
      \csname LTb\endcsname%
      \put(4382,1640){\makebox(0,0)[l]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(4382,1964){\makebox(0,0)[l]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(4382,2288){\makebox(0,0)[l]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(4382,2611){\makebox(0,0)[l]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(4382,2935){\makebox(0,0)[l]{\strut{}$2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_1)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(4984,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_{2,3})/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2513,130){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}}$}}%
      \csname LTb\endcsname%
      \put(3418,2768){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(3418,2582){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(3418,2396){\makebox(0,0)[r]{\strut{}$f_3$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/amplitudes}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/oc-data/oc-obs-model.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2735){\makebox(0,0)[r]{\strut{}$-500$}}%
      \csname LTb\endcsname%
      \put(640,2916){\makebox(0,0)[r]{\strut{}$-400$}}%
      \csname LTb\endcsname%
      \put(640,3097){\makebox(0,0)[r]{\strut{}$-300$}}%
      \csname LTb\endcsname%
      \put(640,3278){\makebox(0,0)[r]{\strut{}$-200$}}%
      \csname LTb\endcsname%
      \put(640,3459){\makebox(0,0)[r]{\strut{}$-100$}}%
      \csname LTb\endcsname%
      \put(640,3640){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,3822){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(640,4003){\makebox(0,0)[r]{\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(640,4184){\makebox(0,0)[r]{\strut{}$300$}}%
      \csname LTb\endcsname%
      \put(640,4365){\makebox(0,0)[r]{\strut{}$400$}}%
      \csname LTb\endcsname%
      \put(640,4546){\makebox(0,0)[r]{\strut{}$500$}}%
      \csname LTb\endcsname%
      \put(640,4727){\makebox(0,0)[r]{\strut{}$600$}}%
      \csname LTb\endcsname%
      \put(816,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1230,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1645,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2059,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2473,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2887,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3302,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3716,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4130,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4544,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1018,4987){\makebox(0,0){\strut{}2001}}%
      \csname LTb\endcsname%
      \put(1321,4987){\makebox(0,0){\strut{}2002}}%
      \csname LTb\endcsname%
      \put(1623,4987){\makebox(0,0){\strut{}2003}}%
      \csname LTb\endcsname%
      \put(1926,4987){\makebox(0,0){\strut{}2004}}%
      \csname LTb\endcsname%
      \put(2229,4987){\makebox(0,0){\strut{}2005}}%
      \csname LTb\endcsname%
      \put(2531,4987){\makebox(0,0){\strut{}2006}}%
      \csname LTb\endcsname%
      \put(2833,4987){\makebox(0,0){\strut{}2007}}%
      \csname LTb\endcsname%
      \put(3137,4987){\makebox(0,0){\strut{}2008}}%
      \csname LTb\endcsname%
      \put(3439,4987){\makebox(0,0){\strut{}2009}}%
      \csname LTb\endcsname%
      \put(3742,4987){\makebox(0,0){\strut{}2010}}%
      \csname LTb\endcsname%
      \put(4044,4987){\makebox(0,0){\strut{}2011}}%
      \csname LTb\endcsname%
      \put(4347,4987){\makebox(0,0){\strut{}2012}}%
      \csname LTb\endcsname%
      \put(4650,4987){\makebox(0,0){\strut{}2013}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(37,3731){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(1122,3274){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(1122,3088){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(1122,2902){\makebox(0,0)[r]{\strut{}$f_3$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,886){\makebox(0,0)[r]{\strut{}$-300$}}%
      \csname LTb\endcsname%
      \put(640,1171){\makebox(0,0)[r]{\strut{}$-200$}}%
      \csname LTb\endcsname%
      \put(640,1455){\makebox(0,0)[r]{\strut{}$-100$}}%
      \csname LTb\endcsname%
      \put(640,1740){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,2024){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(640,2308){\makebox(0,0)[r]{\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(640,2593){\makebox(0,0)[r]{\strut{}$300$}}%
      \csname LTb\endcsname%
      \put(816,484){\makebox(0,0){\strut{}$52000$}}%
      \csname LTb\endcsname%
      \put(1645,484){\makebox(0,0){\strut{}$53000$}}%
      \csname LTb\endcsname%
      \put(2473,484){\makebox(0,0){\strut{}$54000$}}%
      \csname LTb\endcsname%
      \put(3302,484){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(4130,484){\makebox(0,0){\strut{}$56000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(37,1739){\rotatebox{-270}{\makebox(0,0){\strut{}residuals$\unit[/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2804,205){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}-2400000}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{oc-obs-model}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/oc-data/powerspec-planet.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(543,669){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(543,1011){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(543,1354){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(543,1696){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(543,2038){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(543,2380){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(543,2723){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(543,3065){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(719,409){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1162,409){\makebox(0,0){\strut{}$500$}}%
      \csname LTb\endcsname%
      \put(1605,409){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(2047,409){\makebox(0,0){\strut{}$1500$}}%
      \csname LTb\endcsname%
      \put(2490,409){\makebox(0,0){\strut{}$2000$}}%
      \csname LTb\endcsname%
      \put(2933,409){\makebox(0,0){\strut{}$2500$}}%
      \csname LTb\endcsname%
      \put(3376,409){\makebox(0,0){\strut{}$3000$}}%
      \csname LTb\endcsname%
      \put(3819,409){\makebox(0,0){\strut{}$3500$}}%
      \csname LTb\endcsname%
      \put(4262,409){\makebox(0,0){\strut{}$4000$}}%
      \csname LTb\endcsname%
      \put(4704,409){\makebox(0,0){\strut{}$4500$}}%
      \csname LTb\endcsname%
      \put(719,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1126,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1534,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1941,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2349,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2756,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3163,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3571,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3978,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4386,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4793,3139){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1867){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{ltt}/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2756,130){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(4005,2898){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(4005,2712){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(4005,2526){\makebox(0,0)[r]{\strut{}$f_3$}}%
      \csname LTb\endcsname%
      \put(3376,960){\makebox(0,0)[l]{\strut{}$\unit[5]{\sigma}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/oc-data/powerspec-planet}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/powerspec2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(10420.00,7420.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,5286){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,5567){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,5849){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,6130){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(640,6411){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,6692){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(961,7121){\makebox(0,0){\strut{}$-4$}}%
      \csname LTb\endcsname%
      \put(1474,7121){\makebox(0,0){\strut{}$-3$}}%
      \csname LTb\endcsname%
      \put(1987,7121){\makebox(0,0){\strut{}$-2$}}%
      \csname LTb\endcsname%
      \put(2500,7121){\makebox(0,0){\strut{}$-1$}}%
      \csname LTb\endcsname%
      \put(3013,7121){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3525,7121){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(4038,7121){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(4551,7121){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%
      \put(5064,7121){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(5090,6636){\makebox(0,0)[r]{\strut{}2003}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3012,7399){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,3710){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,3991){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,4273){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,4554){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(640,4835){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,5116){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(5090,5060){\makebox(0,0)[r]{\strut{}2008/09}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2134){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,2415){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,2697){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,2978){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(640,3259){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,3540){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(5090,3484){\makebox(0,0)[r]{\strut{}2010}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,839){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,1121){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,1402){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(640,1683){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,1964){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(1232,298){\makebox(0,0){\strut{}$-0.3$}}%
      \csname LTb\endcsname%
      \put(1825,298){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(2419,298){\makebox(0,0){\strut{}$-0.1$}}%
      \csname LTb\endcsname%
      \put(3013,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3606,298){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(4200,298){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4793,298){\makebox(0,0){\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(5090,1908){\makebox(0,0)[r]{\strut{}2011/12}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1345){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(3012,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(9779,5286){\makebox(0,0)[l]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(9779,5601){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(9779,5916){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(9779,6231){\makebox(0,0)[l]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(9779,6546){\makebox(0,0)[l]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(9779,6861){\makebox(0,0)[l]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(5355,7121){\makebox(0,0){\strut{}$-4$}}%
      \csname LTb\endcsname%
      \put(5868,7121){\makebox(0,0){\strut{}$-3$}}%
      \csname LTb\endcsname%
      \put(6381,7121){\makebox(0,0){\strut{}$-2$}}%
      \csname LTb\endcsname%
      \put(6894,7121){\makebox(0,0){\strut{}$-1$}}%
      \csname LTb\endcsname%
      \put(7407,7121){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(7919,7121){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(8432,7121){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(8945,7121){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%
      \put(9458,7121){\makebox(0,0){\strut{}$4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7406,7399){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(9779,5285){\makebox(0,0)[l]{\strut{}}}%
      \csname LTb\endcsname%
      \put(9779,3710){\makebox(0,0)[l]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(9779,4025){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(9779,4340){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(9779,4655){\makebox(0,0)[l]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(9779,4970){\makebox(0,0)[l]{\strut{}$0.8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(9779,3709){\makebox(0,0)[l]{\strut{}}}%
      \csname LTb\endcsname%
      \put(9779,2134){\makebox(0,0)[l]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(9779,2449){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(9779,2764){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(9779,3079){\makebox(0,0)[l]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(9779,3394){\makebox(0,0)[l]{\strut{}$0.8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5626,298){\makebox(0,0){\strut{}$-0.3$}}%
      \csname LTb\endcsname%
      \put(6219,298){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(6813,298){\makebox(0,0){\strut{}$-0.1$}}%
      \csname LTb\endcsname%
      \put(7407,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(8000,298){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(8594,298){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(9187,298){\makebox(0,0){\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(9779,2133){\makebox(0,0)[l]{\strut{}}}%
      \csname LTb\endcsname%
      \put(9779,558){\makebox(0,0)[l]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(9779,873){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(9779,1188){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(9779,1503){\makebox(0,0)[l]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(9779,1818){\makebox(0,0)[l]{\strut{}$0.8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(10304,1345){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(7406,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/powerspec2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/rv/rv.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(766,362){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(1510,362){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(2253,362){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(2996,362){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(3739,362){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(2499,83){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(515,732){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(515,1042){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(515,1352){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(515,1661){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(515,1970){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(515,2280){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(515,2589){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(515,2899){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(184,1893){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[m \sin i/]{M_{\jupiter}}$}}}%
      \csname LTb\endcsname%
      \put(4668,732){\makebox(0,0)[l]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(4668,1184){\makebox(0,0)[l]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(4668,1637){\makebox(0,0)[l]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(4668,2090){\makebox(0,0)[l]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(4668,2542){\makebox(0,0)[l]{\strut{}$16$}}%
      \csname LTb\endcsname%
      \put(4668,2995){\makebox(0,0)[l]{\strut{}$32$}}%
      \csname LTb\endcsname%
      \put(4923,1893){\rotatebox{-270}{\makebox(0,0){\strut{}$\sigma$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/rv/rv}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/window1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1570){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1772){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,1974){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(640,2177){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%
      \put(640,2379){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(640,2581){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \csname LTb\endcsname%
      \put(1446,2841){\makebox(0,0){\strut{}$-0.4$}}%
      \csname LTb\endcsname%
      \put(2151,2841){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(2856,2841){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3560,2841){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4265,2841){\makebox(0,0){\strut{}$0.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,2075){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2855,3119){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1569){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,760){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,962){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1165){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,1367){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(1224,298){\makebox(0,0){\strut{}$-0.04$}}%
      \csname LTb\endcsname%
      \put(2040,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(2856,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3671,298){\makebox(0,0){\strut{}$0.02$}}%
      \csname LTb\endcsname%
      \put(4487,298){\makebox(0,0){\strut{}$0.04$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1063){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(2855,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/window1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/window2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1570){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1959){\makebox(0,0)[r]{\strut{}$0.05$}}%
      \csname LTb\endcsname%
      \put(640,2348){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(1446,2841){\makebox(0,0){\strut{}$-0.4$}}%
      \csname LTb\endcsname%
      \put(2151,2841){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(2856,2841){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3560,2841){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4265,2841){\makebox(0,0){\strut{}$0.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(63,2075){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2855,3119){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1569){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,760){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,962){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1165){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,1367){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(1224,298){\makebox(0,0){\strut{}$-0.04$}}%
      \csname LTb\endcsname%
      \put(2040,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(2856,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3671,298){\makebox(0,0){\strut{}$0.02$}}%
      \csname LTb\endcsname%
      \put(4487,298){\makebox(0,0){\strut{}$0.04$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1063){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(2855,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/window2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/qqvir/window3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1570){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1959){\makebox(0,0)[r]{\strut{}$0.05$}}%
      \csname LTb\endcsname%
      \put(640,2348){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(1446,2841){\makebox(0,0){\strut{}$-0.4$}}%
      \csname LTb\endcsname%
      \put(2151,2841){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(2856,2841){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3560,2841){\makebox(0,0){\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4265,2841){\makebox(0,0){\strut{}$0.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(63,2075){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2855,3119){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1569){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,760){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,962){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1165){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,1367){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(1224,298){\makebox(0,0){\strut{}$-0.04$}}%
      \csname LTb\endcsname%
      \put(2040,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(2856,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3671,298){\makebox(0,0){\strut{}$0.02$}}%
      \csname LTb\endcsname%
      \put(4487,298){\makebox(0,0){\strut{}$0.04$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1063){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(2855,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/qqvir/window3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/sensitive.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(645,1424){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(645,2180){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(821,409){\makebox(0,0){\strut{}$0.01$}}%
      \csname LTb\endcsname%
      \put(2145,409){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(3469,409){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$10$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[m \sin i/]{M_{\jupiter}}$}}}%
      \csname LTb\endcsname%
      \put(2807,130){\makebox(0,0){\strut{}$\unit[a /]{AU}$}}%
      \csname LTb\endcsname%
      \put(1841,1394){\makebox(0,0)[r]{\strut{}DW Lyn}}%
      \csname LTb\endcsname%
      \put(1841,1208){\makebox(0,0)[r]{\strut{}V1636 Ori}}%
      \csname LTb\endcsname%
      \put(1841,1022){\makebox(0,0)[r]{\strut{}QQ Vir}}%
      \csname LTb\endcsname%
      \put(1841,836){\makebox(0,0)[r]{\strut{}V541 Hya}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/sensitive}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/amplitudes.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(645,896){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(645,1122){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(645,1349){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(645,1575){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(645,1802){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(645,2029){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(645,2255){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \csname LTb\endcsname%
      \put(645,2482){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(645,2708){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(1361,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(2037,409){\makebox(0,0){\strut{}$55500$}}%
      \csname LTb\endcsname%
      \put(2713,409){\makebox(0,0){\strut{}$56000$}}%
      \csname LTb\endcsname%
      \put(3388,409){\makebox(0,0){\strut{}$56500$}}%
      \csname LTb\endcsname%
      \put(4064,409){\makebox(0,0){\strut{}$57000$}}%
      \csname LTb\endcsname%
      \put(4510,965){\makebox(0,0)[l]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(4510,1293){\makebox(0,0)[l]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(4510,1621){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4510,1950){\makebox(0,0)[l]{\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(4510,2278){\makebox(0,0)[l]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(4510,2607){\makebox(0,0)[l]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(4510,2935){\makebox(0,0)[l]{\strut{}$0.6$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_1)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(5010,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_2)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2577,130){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}}$}}%
      \csname LTb\endcsname%
      \put(3546,1022){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(3546,836){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/amplitudes}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/lc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5102.00,3152.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,767){\makebox(0,0)[r]{\strut{}0.85}}%
      \put(946,1120){\makebox(0,0)[r]{\strut{}0.90}}%
      \put(946,1474){\makebox(0,0)[r]{\strut{}0.95}}%
      \put(946,1827){\makebox(0,0)[r]{\strut{}1.00}}%
      \put(946,2180){\makebox(0,0)[r]{\strut{}1.05}}%
      \put(946,2534){\makebox(0,0)[r]{\strut{}1.10}}%
      \put(946,2887){\makebox(0,0)[r]{\strut{}1.15}}%
      \put(1141,484){\makebox(0,0){\strut{}$54600$}}%
      \put(1854,484){\makebox(0,0){\strut{}$54800$}}%
      \put(2567,484){\makebox(0,0){\strut{}$55000$}}%
      \put(3279,484){\makebox(0,0){\strut{}$55200$}}%
      \put(3992,484){\makebox(0,0){\strut{}$55400$}}%
      \put(4705,484){\makebox(0,0){\strut{}$55600$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1827){\rotatebox{-270}{\makebox(0,0){\strut{}$Flux$}}}%
      \put(2923,154){\makebox(0,0){\strut{}MBJD(TDB)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/lc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/oc-data/oc-obs-model.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2735){\makebox(0,0)[r]{\strut{}$-50$}}%
      \csname LTb\endcsname%
      \put(640,3188){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,3640){\makebox(0,0)[r]{\strut{}$50$}}%
      \csname LTb\endcsname%
      \put(640,4093){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(640,4546){\makebox(0,0)[r]{\strut{}$150$}}%
      \csname LTb\endcsname%
      \put(1428,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2193,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2957,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3722,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4487,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1123,4987){\makebox(0,0){\strut{}2008}}%
      \csname LTb\endcsname%
      \put(1682,4987){\makebox(0,0){\strut{}2009}}%
      \csname LTb\endcsname%
      \put(2240,4987){\makebox(0,0){\strut{}2010}}%
      \csname LTb\endcsname%
      \put(2798,4987){\makebox(0,0){\strut{}2011}}%
      \csname LTb\endcsname%
      \put(3358,4987){\makebox(0,0){\strut{}2012}}%
      \csname LTb\endcsname%
      \put(3917,4987){\makebox(0,0){\strut{}2013}}%
      \csname LTb\endcsname%
      \put(4475,4987){\makebox(0,0){\strut{}2014}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(139,3731){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(1122,4560){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(1122,4374){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,744){\makebox(0,0)[r]{\strut{}$-100$}}%
      \csname LTb\endcsname%
      \put(640,1197){\makebox(0,0)[r]{\strut{}$-50$}}%
      \csname LTb\endcsname%
      \put(640,1649){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,2102){\makebox(0,0)[r]{\strut{}$50$}}%
      \csname LTb\endcsname%
      \put(640,2554){\makebox(0,0)[r]{\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(1428,484){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(2193,484){\makebox(0,0){\strut{}$55500$}}%
      \csname LTb\endcsname%
      \put(2957,484){\makebox(0,0){\strut{}$56000$}}%
      \csname LTb\endcsname%
      \put(3722,484){\makebox(0,0){\strut{}$56500$}}%
      \csname LTb\endcsname%
      \put(4487,484){\makebox(0,0){\strut{}$57000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(37,1739){\rotatebox{-270}{\makebox(0,0){\strut{}residuals$\unit[/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2804,205){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}-2400000}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{oc-obs-model}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/oc-data/powerspec-planet.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(543,669){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(543,935){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%
      \put(543,1201){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(543,1468){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%
      \put(543,1734){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(543,2000){\makebox(0,0)[r]{\strut{}$25$}}%
      \csname LTb\endcsname%
      \put(543,2266){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(543,2533){\makebox(0,0)[r]{\strut{}$35$}}%
      \csname LTb\endcsname%
      \put(543,2799){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(543,3065){\makebox(0,0)[r]{\strut{}$45$}}%
      \csname LTb\endcsname%
      \put(719,409){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1534,409){\makebox(0,0){\strut{}$500$}}%
      \csname LTb\endcsname%
      \put(2349,409){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(3163,409){\makebox(0,0){\strut{}$1500$}}%
      \csname LTb\endcsname%
      \put(3978,409){\makebox(0,0){\strut{}$2000$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$2500$}}%
      \csname LTb\endcsname%
      \put(719,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1534,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2349,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3163,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3978,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4793,3139){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1867){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{ltt}/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2756,130){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(4005,2898){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(4005,2712){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(4467,848){\makebox(0,0)[l]{\strut{}$\unit[5]{\sigma}$}}%
      \csname LTb\endcsname%
      \put(980,2626){\makebox(0,0){\strut{}$\unit[160]{d}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/oc-data/powerspec-planet}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/oc-sim-2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$-50$}}%
      \csname LTb\endcsname%
      \put(645,921){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(645,1173){\makebox(0,0)[r]{\strut{}$-30$}}%
      \csname LTb\endcsname%
      \put(645,1424){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(645,1676){\makebox(0,0)[r]{\strut{}$-10$}}%
      \csname LTb\endcsname%
      \put(645,1928){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(645,2180){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(645,2431){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(645,2683){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(821,409){\makebox(0,0){\strut{}$54600$}}%
      \csname LTb\endcsname%
      \put(1615,409){\makebox(0,0){\strut{}$54800$}}%
      \csname LTb\endcsname%
      \put(2410,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(3204,409){\makebox(0,0){\strut{}$55200$}}%
      \csname LTb\endcsname%
      \put(3999,409){\makebox(0,0){\strut{}$55400$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$55600$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2807,130){\makebox(0,0){\strut{}MBJD(TDB)}}%
      \csname LTb\endcsname%
      \put(4005,1022){\makebox(0,0)[r]{\strut{}$f_{1}$}}%
      \csname LTb\endcsname%
      \put(4005,836){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{oc-sim-2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/oc-sim.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$-50$}}%
      \csname LTb\endcsname%
      \put(645,921){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(645,1173){\makebox(0,0)[r]{\strut{}$-30$}}%
      \csname LTb\endcsname%
      \put(645,1424){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(645,1676){\makebox(0,0)[r]{\strut{}$-10$}}%
      \csname LTb\endcsname%
      \put(645,1928){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(645,2180){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(645,2431){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(645,2683){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(821,409){\makebox(0,0){\strut{}$54600$}}%
      \csname LTb\endcsname%
      \put(1615,409){\makebox(0,0){\strut{}$54800$}}%
      \csname LTb\endcsname%
      \put(2410,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(3204,409){\makebox(0,0){\strut{}$55200$}}%
      \csname LTb\endcsname%
      \put(3999,409){\makebox(0,0){\strut{}$55400$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$55600$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2807,130){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TT}}$}}%
      \csname LTb\endcsname%
      \put(4005,1022){\makebox(0,0)[r]{\strut{}$f_{1.1}$}}%
      \csname LTb\endcsname%
      \put(4005,836){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/oc-sim}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/oc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(645,669){\makebox(0,0)[r]{\strut{}$-50$}}%
      \csname LTb\endcsname%
      \put(645,921){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(645,1173){\makebox(0,0)[r]{\strut{}$-30$}}%
      \csname LTb\endcsname%
      \put(645,1424){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(645,1676){\makebox(0,0)[r]{\strut{}$-10$}}%
      \csname LTb\endcsname%
      \put(645,1928){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(645,2180){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(645,2431){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(645,2683){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(645,2935){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(821,409){\makebox(0,0){\strut{}$54600$}}%
      \csname LTb\endcsname%
      \put(1615,409){\makebox(0,0){\strut{}$54800$}}%
      \csname LTb\endcsname%
      \put(2410,409){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(3204,409){\makebox(0,0){\strut{}$55200$}}%
      \csname LTb\endcsname%
      \put(3999,409){\makebox(0,0){\strut{}$55400$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$55600$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2807,130){\makebox(0,0){\strut{}MBJD(TDB)}}%
      \csname LTb\endcsname%
      \put(4005,1022){\makebox(0,0)[r]{\strut{}$f_{1.1}$}}%
      \csname LTb\endcsname%
      \put(4005,836){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/oc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/rv/rv.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(766,362){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(1554,362){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(2343,362){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(3130,362){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(3918,362){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(2499,83){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(515,732){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(515,1042){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(515,1352){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(515,1661){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(515,1970){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(515,2280){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(515,2589){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(515,2899){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(184,1893){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[m \sin i/]{M_{\jupiter}}$}}}%
      \csname LTb\endcsname%
      \put(4668,732){\makebox(0,0)[l]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(4668,1184){\makebox(0,0)[l]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(4668,1637){\makebox(0,0)[l]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(4668,2090){\makebox(0,0)[l]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(4668,2542){\makebox(0,0)[l]{\strut{}$16$}}%
      \csname LTb\endcsname%
      \put(4668,2995){\makebox(0,0)[l]{\strut{}$32$}}%
      \csname LTb\endcsname%
      \put(4923,1893){\rotatebox{-270}{\makebox(0,0){\strut{}$\sigma$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/rv/rv}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/window1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1570){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1739){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(640,1907){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,2076){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \csname LTb\endcsname%
      \put(640,2244){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,2413){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%
      \put(640,2581){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(1093,2841){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(1534,2841){\makebox(0,0){\strut{}$-0.15$}}%
      \csname LTb\endcsname%
      \put(1974,2841){\makebox(0,0){\strut{}$-0.1$}}%
      \csname LTb\endcsname%
      \put(2415,2841){\makebox(0,0){\strut{}$-0.05$}}%
      \csname LTb\endcsname%
      \put(2856,2841){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3296,2841){\makebox(0,0){\strut{}$0.05$}}%
      \csname LTb\endcsname%
      \put(3737,2841){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(4177,2841){\makebox(0,0){\strut{}$0.15$}}%
      \csname LTb\endcsname%
      \put(4618,2841){\makebox(0,0){\strut{}$0.2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,2075){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2855,3119){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1569){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,760){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,962){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1165){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,1367){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(816,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(1326,298){\makebox(0,0){\strut{}$-0.015$}}%
      \csname LTb\endcsname%
      \put(1836,298){\makebox(0,0){\strut{}$-0.01$}}%
      \csname LTb\endcsname%
      \put(2346,298){\makebox(0,0){\strut{}$-0.005$}}%
      \csname LTb\endcsname%
      \put(2856,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3365,298){\makebox(0,0){\strut{}$0.005$}}%
      \csname LTb\endcsname%
      \put(3875,298){\makebox(0,0){\strut{}$0.01$}}%
      \csname LTb\endcsname%
      \put(4385,298){\makebox(0,0){\strut{}$0.015$}}%
      \csname LTb\endcsname%
      \put(4895,298){\makebox(0,0){\strut{}$0.02$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1063){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(2855,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/window1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v1636ori/window2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1570){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,1974){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(640,2379){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(1093,2841){\makebox(0,0){\strut{}$-0.2$}}%
      \csname LTb\endcsname%
      \put(1534,2841){\makebox(0,0){\strut{}$-0.15$}}%
      \csname LTb\endcsname%
      \put(1974,2841){\makebox(0,0){\strut{}$-0.1$}}%
      \csname LTb\endcsname%
      \put(2415,2841){\makebox(0,0){\strut{}$-0.05$}}%
      \csname LTb\endcsname%
      \put(2856,2841){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3296,2841){\makebox(0,0){\strut{}$0.05$}}%
      \csname LTb\endcsname%
      \put(3737,2841){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(4177,2841){\makebox(0,0){\strut{}$0.15$}}%
      \csname LTb\endcsname%
      \put(4618,2841){\makebox(0,0){\strut{}$0.2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,2075){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{obs}/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2855,3119){\makebox(0,0){\strut{}$\unit[f /]{\mu Hz}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,1569){\makebox(0,0)[r]{\strut{}}}%
      \csname LTb\endcsname%
      \put(640,558){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,760){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(640,962){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(640,1165){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(640,1367){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(816,298){\makebox(0,0){\strut{}$-0.02$}}%
      \csname LTb\endcsname%
      \put(1326,298){\makebox(0,0){\strut{}$-0.015$}}%
      \csname LTb\endcsname%
      \put(1836,298){\makebox(0,0){\strut{}$-0.01$}}%
      \csname LTb\endcsname%
      \put(2346,298){\makebox(0,0){\strut{}$-0.005$}}%
      \csname LTb\endcsname%
      \put(2856,298){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(3365,298){\makebox(0,0){\strut{}$0.005$}}%
      \csname LTb\endcsname%
      \put(3875,298){\makebox(0,0){\strut{}$0.01$}}%
      \csname LTb\endcsname%
      \put(4385,298){\makebox(0,0){\strut{}$0.015$}}%
      \csname LTb\endcsname%
      \put(4895,298){\makebox(0,0){\strut{}$0.02$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(165,1063){\rotatebox{-270}{\makebox(0,0){\strut{}$A_{window}$}}}%
      \csname LTb\endcsname%
      \put(2855,19){\makebox(0,0){\strut{}$\unit[f /]{d^{-1}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v1636ori/window2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v541hya/oc-data/oc-obs-model.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,5100.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,2888){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(640,3195){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(640,3501){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,3808){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(640,4114){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(640,4421){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%
      \put(640,4727){\makebox(0,0)[r]{\strut{}$80$}}%
      \csname LTb\endcsname%
      \put(816,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1258,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1700,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2142,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2584,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3025,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3467,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3909,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4351,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4793,2549){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1116,4987){\makebox(0,0){\strut{}2004}}%
      \csname LTb\endcsname%
      \put(1439,4987){\makebox(0,0){\strut{}2005}}%
      \csname LTb\endcsname%
      \put(1762,4987){\makebox(0,0){\strut{}2006}}%
      \csname LTb\endcsname%
      \put(2084,4987){\makebox(0,0){\strut{}2007}}%
      \csname LTb\endcsname%
      \put(2408,4987){\makebox(0,0){\strut{}2008}}%
      \csname LTb\endcsname%
      \put(2730,4987){\makebox(0,0){\strut{}2009}}%
      \csname LTb\endcsname%
      \put(3053,4987){\makebox(0,0){\strut{}2010}}%
      \csname LTb\endcsname%
      \put(3375,4987){\makebox(0,0){\strut{}2011}}%
      \csname LTb\endcsname%
      \put(3699,4987){\makebox(0,0){\strut{}2012}}%
      \csname LTb\endcsname%
      \put(4021,4987){\makebox(0,0){\strut{}2013}}%
      \csname LTb\endcsname%
      \put(4344,4987){\makebox(0,0){\strut{}2014}}%
      \csname LTb\endcsname%
      \put(4667,4987){\makebox(0,0){\strut{}2015}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(139,3731){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[(O-C)/]{s}$}}}%
      \csname LTb\endcsname%
      \put(1122,4560){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(1122,4374){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(640,897){\makebox(0,0)[r]{\strut{}$-60$}}%
      \csname LTb\endcsname%
      \put(640,1203){\makebox(0,0)[r]{\strut{}$-40$}}%
      \csname LTb\endcsname%
      \put(640,1510){\makebox(0,0)[r]{\strut{}$-20$}}%
      \csname LTb\endcsname%
      \put(640,1816){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(640,2122){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(640,2429){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(640,2735){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%
      \put(816,484){\makebox(0,0){\strut{}$53000$}}%
      \csname LTb\endcsname%
      \put(1258,484){\makebox(0,0){\strut{}$53500$}}%
      \csname LTb\endcsname%
      \put(1700,484){\makebox(0,0){\strut{}$54000$}}%
      \csname LTb\endcsname%
      \put(2142,484){\makebox(0,0){\strut{}$54500$}}%
      \csname LTb\endcsname%
      \put(2584,484){\makebox(0,0){\strut{}$55000$}}%
      \csname LTb\endcsname%
      \put(3025,484){\makebox(0,0){\strut{}$55500$}}%
      \csname LTb\endcsname%
      \put(3467,484){\makebox(0,0){\strut{}$56000$}}%
      \csname LTb\endcsname%
      \put(3909,484){\makebox(0,0){\strut{}$56500$}}%
      \csname LTb\endcsname%
      \put(4351,484){\makebox(0,0){\strut{}$57000$}}%
      \csname LTb\endcsname%
      \put(4793,484){\makebox(0,0){\strut{}$57500$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(139,1739){\rotatebox{-270}{\makebox(0,0){\strut{}residuals$\unit[/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2804,205){\makebox(0,0){\strut{}$\unit[t/]{MBJD_{TDB}-2400000}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{oc-obs-model}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v541hya/oc-data/powerspec-planet.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(543,669){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(543,1011){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(543,1354){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(543,1696){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(543,2038){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(543,2380){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(543,2723){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(543,3065){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(719,409){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1228,409){\makebox(0,0){\strut{}$500$}}%
      \csname LTb\endcsname%
      \put(1738,409){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(2247,409){\makebox(0,0){\strut{}$1500$}}%
      \csname LTb\endcsname%
      \put(2756,409){\makebox(0,0){\strut{}$2000$}}%
      \csname LTb\endcsname%
      \put(3265,409){\makebox(0,0){\strut{}$2500$}}%
      \csname LTb\endcsname%
      \put(3775,409){\makebox(0,0){\strut{}$3000$}}%
      \csname LTb\endcsname%
      \put(4284,409){\makebox(0,0){\strut{}$3500$}}%
      \csname LTb\endcsname%
      \put(4793,409){\makebox(0,0){\strut{}$4000$}}%
      \csname LTb\endcsname%
      \put(719,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1228,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1738,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2247,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2756,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3265,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3775,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4284,3139){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(4793,3139){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1867){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A_{ltt}/]{s}$}}}%
      \csname LTb\endcsname%
      \put(2756,130){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(4005,2898){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(4005,2712){\makebox(0,0)[r]{\strut{}$f_2$}}%
      \csname LTb\endcsname%
      \put(4487,1113){\makebox(0,0)[l]{\strut{}$\unit[5]{\sigma}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v541hya/oc-data/powerspec-planet}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/exotime/v541hya/rv/rv.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(766,362){\makebox(0,0){\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(1519,362){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(2273,362){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(3025,362){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(3778,362){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%
      \put(2499,83){\makebox(0,0){\strut{}$\unit[P/]{d}$}}%
      \csname LTb\endcsname%
      \put(515,732){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(515,1042){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(515,1352){\makebox(0,0)[r]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(515,1661){\makebox(0,0)[r]{\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(515,1970){\makebox(0,0)[r]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(515,2280){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(515,2589){\makebox(0,0)[r]{\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(515,2899){\makebox(0,0)[r]{\strut{}$14$}}%
      \csname LTb\endcsname%
      \put(184,1893){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[m \sin i/]{M_{\jupiter}}$}}}%
      \csname LTb\endcsname%
      \put(4668,732){\makebox(0,0)[l]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(4668,1184){\makebox(0,0)[l]{\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(4668,1637){\makebox(0,0)[l]{\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(4668,2090){\makebox(0,0)[l]{\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(4668,2542){\makebox(0,0)[l]{\strut{}$16$}}%
      \csname LTb\endcsname%
      \put(4668,2995){\makebox(0,0)[l]{\strut{}$32$}}%
      \csname LTb\endcsname%
      \put(4923,1893){\rotatebox{-270}{\makebox(0,0){\strut{}$\sigma$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/v541hya/rv/rv}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/kepler/KIC7917485/oc-data/amplitudes.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5100.00,3140.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(747,669){\makebox(0,0)[r]{\strut{}0.39}}%
      \csname LTb\endcsname%
      \put(747,1424){\makebox(0,0)[r]{\strut{}0.40}}%
      \csname LTb\endcsname%
      \put(747,2180){\makebox(0,0)[r]{\strut{}0.41}}%
      \csname LTb\endcsname%
      \put(747,2935){\makebox(0,0)[r]{\strut{}0.42}}%
      \csname LTb\endcsname%
      \put(1312,409){\makebox(0,0){\strut{}$5000$}}%
      \csname LTb\endcsname%
      \put(2286,409){\makebox(0,0){\strut{}$5500$}}%
      \csname LTb\endcsname%
      \put(3259,409){\makebox(0,0){\strut{}$6000$}}%
      \csname LTb\endcsname%
      \put(4232,409){\makebox(0,0){\strut{}$6500$}}%
      \csname LTb\endcsname%
      \put(4408,669){\makebox(0,0)[l]{\strut{}$0.19$}}%
      \csname LTb\endcsname%
      \put(4408,1122){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(4408,1575){\makebox(0,0)[l]{\strut{}$0.21$}}%
      \csname LTb\endcsname%
      \put(4408,2029){\makebox(0,0)[l]{\strut{}$0.22$}}%
      \csname LTb\endcsname%
      \put(4408,2482){\makebox(0,0)[l]{\strut{}$0.23$}}%
      \csname LTb\endcsname%
      \put(4408,2935){\makebox(0,0)[l]{\strut{}$0.24$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(144,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_1)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(5010,1802){\rotatebox{-270}{\makebox(0,0){\strut{}$\unit[A(f_2)/]{\%}$}}}%
      \csname LTb\endcsname%
      \put(2577,130){\makebox(0,0){\strut{}$\unit[t/]{BJD_{TDB}-2450000}$}}%
      \csname LTb\endcsname%
      \put(1229,1022){\makebox(0,0)[r]{\strut{}$f_1$}}%
      \csname LTb\endcsname%
      \put(1229,836){\makebox(0,0)[r]{\strut{}$f_2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/KIC7917485/oc-data/amplitudes}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/pipeline/ltt_orbit/drawing.tex <==
%LaTeX with PSTricks extensions
%%Creator: inkscape 0.91
%%Please note this file requires PSTricks extensions
\psset{xunit=.5pt,yunit=.5pt,runit=.5pt}
\begin{pspicture}(531.89998627,328.50000858)
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2.39999974,linecolor=curcolor]
{
\newpath
\moveto(493.50805885,175.17609351)
\curveto(493.50805885,122.15676703)(393.21985471,79.17611068)(269.50808555,79.17611068)
\curveto(145.79631638,79.17611068)(45.50811225,122.15676703)(45.50811225,175.17609351)
\curveto(45.50811225,228.19542)(145.79631638,271.17607635)(269.50808555,271.17607635)
\curveto(393.21985471,271.17607635)(493.50805885,228.19542)(493.50805885,175.17609351)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2.39999974,linecolor=curcolor]
{
\newpath
\moveto(381.5080722,175.17609351)
\curveto(381.5080722,148.66643027)(331.36397013,127.1761021)(269.50808555,127.1761021)
\curveto(207.65220096,127.1761021)(157.5080989,148.66643027)(157.5080989,175.17609351)
\curveto(157.5080989,201.68575676)(207.65220096,223.17608493)(269.50808555,223.17608493)
\curveto(331.36397013,223.17608493)(381.5080722,201.68575676)(381.5080722,175.17609351)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(413.50806838,415.17598956)
\lineto(429.50806647,415.17598956)
\lineto(429.50806647,383.17599529)
\lineto(413.50806838,383.17599529)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2.39999974,linecolor=curcolor]
{
\newpath
\moveto(413.50806838,415.17598956)
\lineto(429.50806647,415.17598956)
\lineto(429.50806647,383.17599529)
\lineto(413.50806838,383.17599529)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(539.99993608,679.99994771)
\lineto(462.97136295,716.03768113)
\lineto(389.61566197,673.01372753)
\lineto(400.08644707,757.40852165)
\lineto(336.50007496,813.87880208)
\lineto(419.99994917,829.9999199)
\lineto(454.05711097,907.92442617)
\lineto(495.19208619,833.4930308)
\lineto(579.82694185,825.18274379)
\lineto(521.74988045,763.0604938)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(579.99993103,759.99994852)
\lineto(496.93937872,778.25000218)
\lineto(434.81712657,720.17294414)
\lineto(426.50683784,804.80779569)
\lineto(352.0754384,845.94276696)
\lineto(429.99994983,879.99992818)
\lineto(446.12106729,963.4997966)
\lineto(502.59135264,899.91342825)
\lineto(586.9861506,910.38421371)
\lineto(543.96219488,837.02851563)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(397.50807072,415.17598956)
\lineto(402.21035172,405.64812724)
\lineto(412.72497287,404.12026304)
\lineto(405.11652152,396.70385694)
\lineto(406.91263286,386.23172258)
\lineto(397.50807032,391.17599386)
\lineto(388.10350703,386.23172308)
\lineto(389.89961908,396.70385688)
\lineto(382.29116797,404.12026386)
\lineto(392.80578881,405.6481272)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(519.99993508,779.99994407)
\lineto(484.57870189,821.76140507)
\lineto(430.0957658,816.25745094)
\lineto(458.86751476,862.85004474)
\lineto(436.79678985,912.96557768)
\lineto(489.99994182,899.99992327)
\lineto(530.84241976,936.47698013)
\lineto(534.95202702,881.87117122)
\lineto(582.26479149,854.29969922)
\lineto(531.60151648,833.51710774)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(559.99992956,779.99994108)
\lineto(439.99994491,799.99993402)
\lineto(395.79599603,753.99260068)
\lineto(377.7350862,874.29969894)
\lineto(320.31973799,902.12310219)
\lineto(429.15746649,956.47698506)
\lineto(437.87677871,1019.6801273)
\lineto(523.20310402,932.96557607)
\lineto(586.00728353,944.20386292)
\lineto(529.9041242,836.25744007)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(173.50809955,255.17602295)
\lineto(130.0876945,274.80236566)
\lineto(109.90711712,231.63676482)
\lineto(115.15523629,278.99689496)
\lineto(67.86616652,284.85085921)
\lineto(114.53008759,294.49468663)
\lineto(105.48441256,341.27823634)
\lineto(129.07618266,299.87831935)
\lineto(170.77471781,322.93817893)
\lineto(138.69131252,287.70779567)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(467.09242402,432.91945563)
\curveto(467.09242402,417.64629606)(441.84419478,405.26495389)(410.69892565,405.26495389)
\curveto(379.55365652,405.26495389)(354.30542728,417.64629606)(354.30542728,432.91945563)
\curveto(354.30542728,448.1926152)(379.55365652,460.57395737)(410.69892565,460.57395737)
\curveto(441.84419478,460.57395737)(467.09242402,448.1926152)(467.09242402,432.91945563)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2.39999974,linecolor=curcolor]
{
\newpath
\moveto(467.09242402,432.91945563)
\curveto(467.09242402,417.64629606)(441.84419478,405.26495389)(410.69892565,405.26495389)
\curveto(379.55365652,405.26495389)(354.30542728,417.64629606)(354.30542728,432.91945563)
\curveto(354.30542728,448.1926152)(379.55365652,460.57395737)(410.69892565,460.57395737)
\curveto(441.84419478,460.57395737)(467.09242402,448.1926152)(467.09242402,432.91945563)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2.39999974,linecolor=curcolor]
{
\newpath
\moveto(198.54739305,135.44074407)
\lineto(180.75687102,137.15788602)
\lineto(168.37097867,124.27220258)
\lineto(164.50650417,141.72261952)
\lineto(148.42403901,149.52040728)
\lineto(163.82618445,158.58821611)
\lineto(166.2725667,176.29319742)
\lineto(179.65609058,164.44699454)
\lineto(197.25050312,167.59148701)
\lineto(190.11983034,151.20232216)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=2.39999974,linecolor=curcolor]
{
\newpath
\moveto(468.89593413,235.51168332)
\curveto(473.23830319,227.99048012)(470.66134859,218.37315479)(463.14014494,214.03078599)
\curveto(455.61894128,209.68841719)(446.00161538,212.26537163)(441.65924632,219.78657484)
\curveto(437.31687726,227.30777804)(439.89383186,236.92510337)(447.41503552,241.26747217)
\curveto(454.93623917,245.60984097)(464.55356507,243.03288653)(468.89593413,235.51168332)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.05098039 0.05098039 1}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(279.13910499,166.67466095)
\lineto(270.04279472,175.77097019)
\lineto(260.94648876,166.67466046)
\lineto(270.04279854,175.77097019)
\lineto(260.94648827,184.86727561)
\lineto(270.04279854,175.77096636)
\lineto(279.1391045,184.86727609)
\lineto(270.04279472,175.77096636)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.59999982,linecolor=curcolor]
{
\newpath
\moveto(279.13910499,166.67466095)
\lineto(270.04279472,175.77097019)
\lineto(260.94648876,166.67466046)
\lineto(270.04279854,175.77097019)
\lineto(260.94648827,184.86727561)
\lineto(270.04279854,175.77096636)
\lineto(279.1391045,184.86727609)
\lineto(270.04279472,175.77096636)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.59999979,linecolor=curcolor,linestyle=dashed,dash=9.6 9.6]
{
\newpath
\moveto(269.50807787,175.17603074)
\lineto(269.50807787,36.64797551)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.59999979,linecolor=curcolor,linestyle=dashed,dash=9.6 9.6]
{
\newpath
\moveto(175.67871906,149.96486525)
\curveto(175.3587891,8.42538056)(175.67871906,12.86727976)(175.67871906,12.86727976)
\lineto(175.67871906,12.86727976)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.59999979,linecolor=curcolor,linestyle=dashed,dash=9.6 9.6]
{
\newpath
\moveto(455.5358257,228.33112124)
\lineto(455.5358257,87.15100648)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.55403996,linecolor=curcolor]
{
\newpath
\moveto(272.6234775,39.14927506)
\lineto(453.31491596,89.19376612)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(278.614119,40.80844944)
\lineto(280.77985252,44.6333572)
\lineto(271.12581713,38.73448147)
\lineto(282.43902699,38.64271606)
\lineto(278.614119,40.80844944)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=0.77701998,linecolor=curcolor]
{
\newpath
\moveto(278.614119,40.80844944)
\lineto(280.77985252,44.6333572)
\lineto(271.12581713,38.73448147)
\lineto(282.43902699,38.64271606)
\lineto(278.614119,40.80844944)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(447.32427446,87.53459174)
\lineto(445.15854095,83.70968398)
\lineto(454.81257634,89.60855971)
\lineto(443.49936647,89.70032512)
\lineto(447.32427446,87.53459174)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=0.77701998,linecolor=curcolor]
{
\newpath
\moveto(447.32427446,87.53459174)
\lineto(445.15854095,83.70968398)
\lineto(454.81257634,89.60855971)
\lineto(443.49936647,89.70032512)
\lineto(447.32427446,87.53459174)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.51906778,linecolor=curcolor]
{
\newpath
\moveto(178.38615873,13.2183797)
\lineto(267.50243811,37.90027529)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(184.24198392,14.84022553)
\lineto(186.35897355,18.57906086)
\lineto(176.92220244,12.81291824)
\lineto(187.98081947,12.72323602)
\lineto(184.24198392,14.84022553)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=0.75953389,linecolor=curcolor]
{
\newpath
\moveto(184.24198392,14.84022553)
\lineto(186.35897355,18.57906086)
\lineto(176.92220244,12.81291824)
\lineto(187.98081947,12.72323602)
\lineto(184.24198392,14.84022553)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(261.64661293,36.27842946)
\lineto(259.5296233,32.53959413)
\lineto(268.96639441,38.30573674)
\lineto(257.90777738,38.39541897)
\lineto(261.64661293,36.27842946)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=0.75953389,linecolor=curcolor]
{
\newpath
\moveto(261.64661293,36.27842946)
\lineto(259.5296233,32.53959413)
\lineto(268.96639441,38.30573674)
\lineto(257.90777738,38.39541897)
\lineto(261.64661293,36.27842946)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=1.99999994,linecolor=curcolor,linestyle=dashed,dash=2.0000003 8.00000119]
{
\newpath
\moveto(268.80312796,176.82512045)
\curveto(422.7608096,321.78869452)(423.28986954,322.31776443)(423.28986954,322.31776443)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linewidth=0.79999989,linecolor=curcolor]
{
\newpath
\moveto(400.33720228,301.05739823)
\curveto(421.75328972,279.39374211)(406.23941157,251.39020711)(406.23941157,251.39020711)
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(144.79844503,139.03092903)
\lineto(147.73789836,139.03092903)
\lineto(151.45860175,129.10905391)
\lineto(155.1988364,139.03092903)
\lineto(158.13828973,139.03092903)
\lineto(158.13828973,124.45085073)
\lineto(156.21446147,124.45085073)
\lineto(156.21446147,137.25358526)
\lineto(152.45469557,127.25358514)
\lineto(150.47227356,127.25358514)
\lineto(146.71250766,137.25358526)
\lineto(146.71250766,124.45085073)
\lineto(144.79844503,124.45085073)
\lineto(144.79844503,139.03092903)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(438.05247052,209.43724927)
\curveto(438.5016893,210.24454095)(439.03879871,210.84024408)(439.66379876,211.22435867)
\curveto(440.2887988,211.60847326)(441.02447594,211.80053055)(441.87083016,211.80053055)
\curveto(443.01015316,211.80053055)(443.88905947,211.40013992)(444.5075491,210.59935866)
\curveto(445.12603873,209.80508782)(445.43528354,208.6722753)(445.43528354,207.20092112)
\lineto(445.43528354,200.59935854)
\lineto(443.62864279,200.59935854)
\lineto(443.62864279,207.14232737)
\curveto(443.62864279,208.19050446)(443.4430959,208.96849927)(443.07200212,209.47631177)
\curveto(442.70090835,209.98412428)(442.13450206,210.23803053)(441.37278325,210.23803053)
\curveto(440.4417936,210.23803053)(439.70611647,209.92878574)(439.16575185,209.31029614)
\curveto(438.62538722,208.69180655)(438.35520491,207.84870759)(438.35520491,206.78099924)
\lineto(438.35520491,200.59935854)
\lineto(436.54856416,200.59935854)
\lineto(436.54856416,207.14232737)
\curveto(436.54856416,208.19701488)(436.36301727,208.97500968)(435.99192349,209.47631177)
\curveto(435.62082972,209.98412428)(435.04791301,210.23803053)(434.27317337,210.23803053)
\curveto(433.35520455,210.23803053)(432.62603784,209.92553053)(432.08567321,209.30053052)
\curveto(431.54530859,208.68204093)(431.27512628,207.84219717)(431.27512628,206.78099924)
\lineto(431.27512628,200.59935854)
\lineto(429.46848553,200.59935854)
\lineto(429.46848553,211.53685867)
\lineto(431.27512628,211.53685867)
\lineto(431.27512628,209.8376399)
\curveto(431.68528256,210.50821283)(432.17681905,211.0030045)(432.74973576,211.32201492)
\curveto(433.32265247,211.64102534)(434.00299106,211.80053055)(434.79075153,211.80053055)
\curveto(435.58502242,211.80053055)(436.2588506,211.59870763)(436.81223605,211.19506179)
\curveto(437.37213193,210.79141595)(437.78554341,210.20547845)(438.05247052,209.43724927)
\closepath
}
}
\end{pspicture}


==> preamble/preamble.tex <==
\usepackage[automark]{scrlayer-scrpage}
\usepackage[ngerman,english,greek]{babel}
\usepackage{textgreek}
%\usepackage[onehalfspacing]{setspace}		%Zeilenabstand, für Titelseite auf 1 setzen!
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{lmodern}
\usepackage[
	autostyle=true,
	english=british
]{csquotes}
\usepackage{scrextend}

\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{color}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows,shapes.multipart,positioning,fit,calc}

\usepackage{wrapfig}
\usepackage{subcaption}
\usepackage{longtable}
\usepackage{pdflscape}
\usepackage[percent]{overpic}
\usepackage{epstopdf}
\usepackage{adjustbox}
\usepackage{booktabs}		%Linien für Tabellen
\usepackage{gensymb}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{wasysym}

\usepackage[ugly]{units}
\usepackage{siunitx}
\DeclareSIUnit\au{au}

\usepackage{listings}
\lstset{breaklines=true,                 % sets automatic line breaking
%	numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
	tabsize=2,	                   % sets default tabsize to 2 spaces
}
% for correct line-numbering in listings:
\makeatletter
% http://tex.stackexchange.com/q/26828/5764
\patchcmd{\lst@GLI@}% <command>
{\def\lst@firstline{#1\relax}}% <search>
{\def\lst@firstline{#1\relax}\def\lst@firstnumber{#1\relax}}% <replace>
{\typeout{listings firstnumber=firstline}}% <success>
{\typeout{listings firstnumber not set}}% <failure>
\makeatother
%----------

\usepackage[
	%dvipdfm,
	colorlinks=true,
	linkcolor=black,
	citecolor=black,
	filecolor=black,
	urlcolor=black,
	bookmarks=true,
	bookmarksopen=true,
	bookmarksopenlevel=3,
	plainpages=false,
	pdfpagelabels=true
	pdftitle={Dissertation zur Erlangung des mathematisch-naturwissenschaftlichen Doktorgrades zur Erlangung des Doktorgrades},
	pdfsubject={Title},
	pdfauthor={Felix Mackebrandt},
	pdflang=en,
	pdfdisplaydoctitle=true
]{hyperref}
\usepackage[hypcap]{caption}
\usepackage{blindtext}

%\usepackage[authoryear,
%round,
%sort&compress,
%nonamebreak
%]{natbib}

\usepackage{natbib}
\bibpunct{(}{)}{;}{a}{}{,}	% to follow the A&A style


\hyphenation{
mol-e-cules
}

\newcommand{\diff}[2]{\frac{\mathrm{d}#1}{\mathrm{d}#2}}
\newcommand{\dif}[1]{\mathrm{d}#1}
%\allowdisplaybreaks %align über mehrere Seiten

